Blending Data-Driven Priors in Dynamic Games

As intelligent robots like autonomous vehicles become increasingly deployed in the presence of people, the extent to which these systems should leverage model-based game-theoretic planners versus data-driven policies for safe, interaction-aware motion planning remains an open question. Existing dynamic game formulations assume all agents are task-driven and behave optimally. However, in reality, humans tend to deviate from the decisions prescribed by these models, and their behavior is better approximated under a noisy-rational paradigm. In this work, we investigate a principled methodology to blend a data-driven reference policy with an optimization-based game-theoretic policy. We formulate KLGame, an algorithm for solving non-cooperative dynamic game with Kullback-Leibler (KL) regularization with respect to a general, stochastic, and possibly multi-modal reference policy. Our method incorporates, for each decision maker, a tunable parameter that permits modulation between task-driven and data-driven behaviors. We propose an efficient algorithm for computing multi-modal approximate feedback Nash equilibrium strategies of KLGame in real time. Through a series of simulated and real-world autonomous driving scenarios, we demonstrate that KLGame policies can more effectively incorporate guidance from the reference policy and account for noisily-rational human behaviors versus non-regularized baselines. Website with additional information, videos, and code: https://kl-games.github.io/.

==> rebuttal/statement_of_changes.tex <==


\onecolumn

\section*{Our Meta Comments}
We sincerely thank the reviewers and the Area Chair for their detailed feedback. We are happy to see that the reviewers appreciated (1). the strong motivation for combining data-driven and model-based planning approaches in challenging settings (potentially beyond our application domain of autonomous driving) (2). the intuitive theoretical approach of the framework, and (3). the effective application in several settings in both simulation and hardware. In response to the reviewers’ concerns and suggestions, we have made appropriate changes to the paper and performed new experiments as summarized below. We address the main concerns first, and we then respond to individual reviewers. For convenience, we have attached the revised manuscript to this document, with changes highlighted in \rebuttal{blue color}.

\vspace{0.2cm}
\section*{Summary of Major Changes}
\noindent 
\textbf{Changes addressing mathematical jargon and accessibility of notation:}
\begin{enumerate}
    \item We have added a notation paragraph at the beginning of Section \ref{sec:problem_formulation} to introduce some of the symbols, e.g., $[T]$. 
    \item We have added a more detailed introduction to the parameters of the model-based optimization in Section \ref{subsec:DPformulation}: the dynamics ($A$ and $B$), the costs ($Q$ and $R$), the reference policy ($\Tilde{\mu}$ and $\Tilde{\Sigma}$).
    \item We have added a paragraph in Section \ref{sec:KLGame} before Theorem \ref{thm:global_nash} to give some insight into where the reader is headed after the notation is introduced. 
\end{enumerate}
\textbf{Changes addressing the need for additional quantitative validation of our approach:}
\begin{enumerate}
    \item We now report the standard deviation for each category in Table \ref{tab: klgame_baseline_comparison} to reflect statistical differences between our method and the baselines used. 
    \item We have added quantitative results for the autonomous racing experiment in Section \ref{subsec:autonomous_car} in Table \ref{tab: racing_stat}, which showcases tangible improvement of the multi-modal KLGame policy over baseline methods in terms of safe rate and overtaking rate, the two critical performance metrics of car racing.
    \item We have added quantitative results for 500 Waymax scenarios from the Waymo open motion dataset (WOMD) Interactive Validation set. We compare our approach against other game-theoretic planning methods such as ILQGames \cite{fridovich2020efficient} as well as MTR, a fully data-driven method \cite{shi2022motion}. We report results in 
    % two tables: Table \ref{tab: waymax_experiment_results_log_replay} compares KLGame to baseline approaches when other agents follow their ground truth (log-replay) trajectories. 
    Table \ref{tab: waymax_experiment_results_idm}, where we compare KLGame to baseline approaches when other agents follow the IDM model, which generates interactive behaviors of the other agents, but is not explicitly modeled in the game-theoretic planner.
\end{enumerate}
\textbf{Changes addressing complexity and scalability of dynamic programming:}
\begin{enumerate}
    \item We have provided a runtime complexity analysis for the full scenario-optimization-based approach that describes how our algorithm scales with the number of agents,  the dimension of the state space, the time horizon, and the branching factor of the scenario tree. Overall, our implementation of the uni-modal KLGame attains the same complexity as baseline approaches, e.g. ILQGames \cite{fridovich2020efficient}, despite benefiting greatly from data-driven models, e.g., MTR \cite{shi2022motion}. We report this analysis in Section \ref{subsec:solving_general_KLGame}. 
    \item We have reported empirical worst case runtime as a function of the number of agents $N$ in Figure \ref{fig:runtime}. 
\end{enumerate}
 \textbf{Changes addressing the clarity of the contribution:}
\begin{enumerate}
    \item We have added a paragraph in Section \ref{subseq:multi_modal_motion_prediction} on how our work differs from existing Multi-Modal Multi-Agent prediction approaches. 
    \item We have added a “Key Takeaway” paragraph for each experiment to provide additional interpretation of the qualitative results from the original submission as well as the new quantitative results. 
\end{enumerate}
\textbf{Changes addressing Figure \ref{fig: Rollouts}:}
\begin{enumerate}
    \item We have changed Figure \ref{fig: Rollouts} to reflect a real scenario from the WOMD dataset, which we model and solve using KLGame in Section \ref{subsec:waymax} 
\end{enumerate}



\vspace{0.2cm}
\section*{Area Chair’s Comments}

\noindent
\emph{All the Reviewers agree that the paper is generally well written, even though the math is quite hard to follow, at some points: this is partially due to the use of (not well defined) jargon and symbols. Authors are then requested to polish the description, and ensure consistency.}
% \textbf{Concern on the mathematical accessibility of the paper and use of jargon.}
\begin{itemize}
    \item We thank the Area Chair for acknowledging the writing quality of our paper. We have added a notation paragraph at the beginning of Section \ref{sec:problem_formulation} to introduce some of the symbols, e.g., $[T]$. Furthermore, we have added a paragraph in Section \ref{sec:KLGame} before Theorem \ref{thm:global_nash} to give some insight into where the reader is headed after the notation is introduced.  With the added changes, along with stating the goal (before stating our main result in Theorem~\ref{thm:global_nash}) of introducing these symbols, we hope that the notational burden has been alleviated.
\end{itemize}


\vspace{0.25cm}
\noindent
\emph{The weakest point of this paper is in the validation of the method, and comparison with the literature. Authors should put effort in clearly showcasing the advantages of the proposed method.}
% \textbf{Concern on the need for additional quantitative validation of our approach.}

\begin{itemize}
    \item We have provided additional experimental results for Toll Booth Coordination (Section \ref{subsec:twoplayertollbooth}), Autonomous Racing (Section \ref{subsec:autonomous_car}) and Waymo (Section \ref{subsec:waymax}).
    \item First, in the original submission, we did not report variance for our Toll Booth results. Now, we show that our method outperforms the baselines by a statistically significant amount, exceeding baseline performance by three standard deviations for some metrics.
    \item In the autonomous racing example, we now report safe rate and overtaking rate results. Compared to the Shielded Inverse Dynamic Game baseline, which explicitly models safety at the expense of limited overtaking ability, our multi-modal KLGame achieves a safe rate of $95\%$ versus $73\%$ for the reference policy. KLGame additionally achieves an overtaking rate of $92\%$ versus $86\%$ for the baseline.
    \item Finally, for our Waymax-based urban driving example, we now report Collision Rates for KLGame against the ILQGames, MaxEnt, intelligent driving model (IDM), and MTR baselines in \cref{tab: waymax_experiment_results_idm}. Specifically, we consider 500 two-agent interactive scenarios selected by \cite{zhang2023cat} from WOMD \cite{ettinger2021waymo}, in which self-driving car (ego) are controlled by each policy and the interacting agents use IDM policy. Overall, KLGame achieves the lowest Collision Rate of {9\%} versus {12\%} for MTR.
\end{itemize}




\vspace{0.2cm}
\section*{Reviewer nSFC’s Comments}

We thank Reviewer nSFC for their thorough and very constructive feedback. In particular, we appreciate the concerns regarding the efficacy of our approach, especially with regard to computational complexity (scaling) and the accuracy of the Laplace approximation. We took note of the suggestions and clarifications, e.g., absolute continuity, and added them to our report. 

\vspace{0.25cm}
\noindent
\emph{The regularization parameter is a heuristic that affects the method’s performance. It seems that the authors selected multiple values of $\lambda$ and presented some extreme cases. Is there a strategy to bound $\lambda$ and ensure safe behavior?}
% \textbf{Concern of the regularization term’s effect on performance:} 
% \noindent \emph{It seems that the control policies in formula (4) is switched (as mentioned in equation 10e). However, the determination of the shielding set should be explained more clearly?}
\begin{itemize}
    \item The regularization term could affect downstream performance for metrics such as safety. However, we would like to clarify that KLGame does not rely on tedious hand tuning of $\lambda$ to perform well. We show in the initial submission (cf. Section \ref{subsec:autonomous_car}) that KLGame performance is robust to the choice of regularization. The regularized game solver allows a robot to balance different objectives (such as finding a natural trajectory subject to safety), and such blending is beneficial for a large range of regularization parameters. 
    \item 
    \looseness=-1
    On finding a strategy to bound $\lambda$: In practice, we observed that KLGame results in safe behaviors for a variety of choices of $\lambda$. A range of valid lambda values can be obtained empirically without a burdensome search; e.g., we tested a spectrum of $\lambda \in [50,50000]$ in the racing example, all leading to safe and successful overtaking. We believe that a theoretically principled procedure for obtaining the exact interval is an interesting area for future work.  
\end{itemize}

\vspace{0.25cm}
\noindent
\emph{A computational complexity analysis is missing. Since DP is computationally expensive, I argue that the scalability is high. Please provide a formal computational complexity analysis..}
% \textbf{Concern on computational complexity:}
\begin{itemize}
    \item We thank the reviewer for bringing up this important point. We note that the DP used for solving KLGame is fundamentally different from grid-based approaches, which are indeed computationally expensive. Similar to the well-known ILQR algorithm, our approach iteratively solves a KL-LQG game, for which the DP solution can be found in closed form via solving the coupled Riccati equation. The computation bottleneck is a matrix inversion operation needed for solving the coupled Riccati equation, which has complexity $\mathcal{O}(N^3n^3)$. Therefore, the overall algorithm scales cubically with the number of agents $N$ and state dimension $n$ and is consistent with other model-based game-theoretic planning approaches, e.g., ILQGames \cite{fridovich2020efficient} but benefits greatly from data-driven models, e.g., MTR \cite{shi2022motion}. We have provided a detailed complexity analysis in Sec.~\ref{subsec:solving_general_KLGame}, accompanied by an empirical study of the algorithm’s computation performance, derived from our experiments.
\end{itemize}

\vspace{0.25cm}
\noindent
\emph{In the second bullet of the contribution you mention that your method is compared with [4]-[6] in Waymo’s open motion dataset, but the comparison is missing. Please elaborate on the comparisons you performed and be consistent throughout the text.}
% \textbf{Concern on quantitative validation on Autonomous Racing and Waymo Open Data Set:}
\begin{itemize}
    \item We have provided additional comparisons to baselines in the Waymo open motion datasets (WOMD). In particular, we now report Collision Rates for KLGame against the ILQGames, MaxEnt, intelligent driving model (IDM), and MTR baselines in \cref{tab: waymax_experiment_results_idm}. Specifically, we consider 500 two-agent interactive scenarios selected by \cite{zhang2023cat} from WOMD \cite{ettinger2021waymo}, in which the self-driving car (ego) are controlled by each policy and the interacting agents use IDM policy. Overall, KLGame achieves the lowest Collision Rate of {9\%} versus {12\%} for MTR.
\end{itemize}

\vspace{0.25cm}
\noindent
\emph{What does absolutely continuous in p. 4 means in technical terms?}
% \textbf{Concern on the definition of absolute continuity:}
\begin{itemize}
    \item We use the standard notation: $\mu << \nu$ (“$\mu$ is absolutely continuous with respect to $\nu$”) if and only if $\mu(A) = 0$ whenever $\nu(A) = 0$ for measurable set $A$. In practice, this is to avoid dividing by zero since the KL divergence uses a probability ratio. We have added the definition in Section \ref{sec:problem_formulation}.
    % $\policy_t^i(\cdot | \jxt)$ is absolutely continuous with respect to $\tilde \pi_t^i(\cdot|\jxt)$ 
\end{itemize}

\vspace{0.25cm}
\noindent
\emph{Why do you use Laplace approximation (LA)? Did you notice any approximation errors? Typically LA is a rough approximation.}
% \textbf{Concern on the use of and accuracy of the Laplace approximation (LA):}
\begin{itemize}
    \item We use LA to approximate arbitrary policy distribution locally as a Gaussian density so that the KLGame is real-time solvable. 
    The approximation errors incurred by the resulting uni-modal Gaussian are partially mitigated by the scenario optimization, which can effectively capture distinct modes of the original policy distribution along different branches of the scenario tree.
    Specifically, we use LA in experiment 2 (racing, Section \ref{subsec:autonomous_car}) to approximate the mean and covariance of the reference policy for each agent, obtained from a small in-house dataset. We conclude from our experiment results that the approximation errors stemming from LA have not notably affected the performance of the KLGame policy. 
\end{itemize}

\vspace{0.25cm}
\noindent
\emph{Please mention throughout the text that your method requires the dynamics to be linearized.}
% \textbf{Concern on linearization:}
\begin{itemize}
    \item Thank you for the suggestion. We have clarified dynamics linearization in the paper. Note that linearized dynamics are only needed in the backward pass of Algorithm \ref{alg:cap}. Then, we simulate the original nonlinear dynamics in the forward pass to update the nominal state and action trajectories.
\end{itemize}

\vspace{0.25cm}
\noindent
\emph{Table I is not informative as std and outliers are not discussed. Please replace it with a box plot.}
% \textbf{Concern on statistical results for Table \ref{tab: klgame_baseline_comparison}:}
\begin{itemize}
    \item Thank you for pointing this out. Since all the metrics we report do not fit on a box plot, we have changed Table \ref{tab: klgame_baseline_comparison} to include one standard deviation. However, we present the results for the racing and Waymax experiments as tables with the mean value alone since they are more extensive numerical studies. 
\end{itemize}


\vspace{0.25cm}
\noindent
\emph{What is the computation time required to implement your method in simulations? Is real-time implementation feasible?}
\begin{itemize}
    \item We have conducted the worst-case computation analysis with respect to various numbers of agents, and the result is shown in Fig.~\ref{fig:runtime}. We repeated each experiment for 80 times and ensure KLGame solver iterates 15 times with 15 line searches. In practice, we observe that Algorithm \ref{alg:cap} typically converges with a small number of iterations and our solver achieves a \textit{10Hz} planning rate for a reasonable number of agents (around four) in complex traffic interaction scenarios (Sec.~\ref{subsec:waymax}) where agents are in close proximity.
    This result indicates that our method is feasible for real-time interactive motion planning.
\end{itemize}

\vspace{0.25cm}
\noindent
\emph{A comparison is provided only in the first simulation. Please compare your method with state-of-the-art methods in the second and third numerical example and discuss the results.
}
\begin{itemize}
    \item We have provided additional experimental results for Autonomous Racing (Section \ref{subsec:autonomous_car}) and Waymo (Section \ref{subsec:waymax}).
    \item In the autonomous racing example, we now report safe rate and overtaking rate results. Compared to the Shielded Inverse Dynamic Game baseline, which explicitly models safety at the expense of limited overtaking ability, our multi-modal KLGame achieves a safe rate of $95\%$ versus $73\%$ for the reference policy. KLGame additionally achieves an overtaking rate of $92\%$ versus $86\%$ for the baseline.
    \item For our Waymax-based urban driving example, we now report Collision Rates for KLGame against the ILQGames, MaxEnt, intelligent driving model (IDM), and MTR baselines in \cref{tab: waymax_experiment_results_idm}. Specifically, we consider 500 two-agent interactive scenarios selected by \cite{zhang2023cat} from WOMD \cite{ettinger2021waymo}, in which self-driving car (ego) are controlled by each policy and the interacting agents use IDM policy. Overall, KLGame achieves the lowest Collision Rate of {9\%} versus {12\%} for MTR.
\end{itemize}


\vspace{0.25cm}
\noindent
\emph{What happens if the network size increases? All numerical examples consider the case of only two vehicles.}
\begin{itemize}
    \item We assume that by network size, the reviewer means the number of agents in the game. If this is the case, we invite the reviewer to read our response to the concern on the computation complexity of our method. We note that the KLGame solution procedure (Alg.~\ref{alg:cap}) is agnostic to the neural network size of the reference policy.
    \item We have added multi-vehicle experiments (up to $14$ interacting agents) in Sec.~\ref{subsec:waymax} and conducted the worst-case computation analysis with respect to various number of agents (Fig.~\ref{fig:runtime}).
\end{itemize}




\vspace{0.2cm}
\section*{Reviewer ZAc5’s Comments}
We thank Reviewer ZAc5 for their constructive and supportive comments on our manuscript. We appreciate that you think our work is insightful and provides a good overview of related work. We acknowledge the previous submission's limitation in statistical validation and sought to rectify these issues by providing additional quantitative comparisons. Moreover, we discuss below the concerns about performance with nonlinear dynamics and multimodality. 

\vspace{0.25cm}
\noindent
\emph{One major limitation of the work is the limited validation. There are three experiments, but only the first one (a toy example) actually compares to some baseline methods in a statistical meaningful way. The other two experiments seem to be a proof-of-concept, demonstrating that KLGame can produce better solutions, but not including any statistical validation.}
% \textbf{Concern on statistical validation:}
\begin{itemize}
    \item Thank you for the feedback.
    This comment relates to that raised by the Area Chair and Reviewer nSFC. We invite the reviewer to consider our answer to that comment in conjunction with what follows.
    We have provided additional validation on the racing and Waymax experiments.
    Specifically, in the racing example, we now report safe rate and overtaking rate results in \cref{tab: racing_stat}.
    For our Waymax-based urban driving example, we now report Collision Rates for KLGame against the ILQGames, MaxEnt, intelligent driving model (IDM), and MTR baselines in \cref{tab: waymax_experiment_results_idm}.
\end{itemize}


\vspace{0.25cm}
\noindent
\emph{Some of the key claims are not properly validated. For example, it remains unclear to what extent the extensions can handle non-linear dynamics and multi-modal distributions. (Only one dynamical system, a 4D kinematic bicycle, was used and it remains unclear how many modes the reference trajectories truly had.) Some of the extensions using linearization are common in other robotic areas and tend to not work well on highly nonlinear systems.}
% \textbf{Concern on more complex dynamics and costs:}
\begin{itemize}
    \item On nonlinearity: We use a 4D kinematic bicycle for all systems. However, this does not preclude our method from being used on highly nonlinear systems. In Sec.~\ref{subsec:waymax}, we applied KLGame to settings where the other agents followed their ground-truth nonlinear dynamics (unknown to the planner), and observed superior performance compared to the MTR baseline. This indicates that KLGame can robustly handle a reasonable level of modeling error during complex interactions. 
    \item On multi-modality: We use a multi-modal reference distribution in the racing and Waymax examples. In racing, the reference policy has two modes: overtaking and car-following. In Waymax, the reference policy has six modes corresponding to the data-driven rollouts.
\end{itemize}

\vspace{0.25cm}
\noindent
\emph{The paper is well written but seems rather long and is not very focused on making a clear contribution. For a conference paper, it might have been better to focus on the linear case only and make a stronger empirical argument in such a setting.}
% \textbf{Potential Concern on Figure 1:}
\begin{itemize}
    \item We are happy to hear that the reviewer found our paper well written. On the concern of contribution: We maintain that are contributions are as stated in the last paragraph in the Introduction:
    \begin{itemize}
        \item We provide a formulation of a new type of dynamic game featuring KL regularization with arbitrary reference distributions that are obtained from data.
        \item We provide an efficient way for solving the dynamic game with KL regularization, with theoretical guarantees.
    \end{itemize}
    Furthermore, we have provided additional wording in each section to keep the message consistent. 
    \item On making a better empirical argument: We back up these claims in three experimental settings, which we now augment with additional empirical results (see e.g. Tables \ref{tab: racing_stat} and \ref{tab: waymax_experiment_results_idm}). At the end of each experiment section, we added a \textbf{Key Takeaway} paragraph to summarize and highlight a specific advantage that our approach offers. We also acknowledge that only focusing on the linear case could potentially limit our contributions to the broader robotics community.
\end{itemize}

\vspace{0.25cm}
\noindent
\emph{Whats the difference between bottom row middle and right picture?}
% \textbf{Potential Concern on Figure 1:}
\begin{itemize}
    \item We are not sure which picture the reviewer is referring to in their original comment, but we will posit that they mean Figure \ref{fig: Rollouts}. We have changed Figure \ref{fig: Rollouts} to be more illustrative of the KLGame spectrum of policies (interpolating between task- and data-optimal) in real-world scenarios by using an example scene from Waymax. 
\end{itemize}


\vspace{0.25cm}
\noindent
\emph{Minor:
\begin{itemize}
    \item "Herein, we use $i$ to denote" is mentioned twice.
    \item Color in (8), (9), (10) unclear.
    \item Some of the paper heavily relies on related work such as [1], [4], [5] and some more detailed background would have been helpful. "Planning Porblems" spelling
\end{itemize}
}

\noindent We have fixed all these issues. Thank you for spotting them!




\vspace{0.2cm}
\section*{Reviewer feC9’s Comments}
We thank the reviewer for providing a set of constructive comments for our paper. We are glad to hear that you think the blending of task-driven and data-driven policies is interesting and that the simulations illustrate the merit of our approach. We have addressed your main concerns and recommendations below, with particular emphasis placed on excessive mathematical notation and jargon; we hope you find our updates helpful.

\vspace{0.25cm}
\noindent
\emph{The equations in the paper are difficult to follow when reading for the first time. Several symbols are not defined within the paper (e.g. $A$, $B$, $K$, $Q$, $R$, $Z$ in Theorem 1). These symbols may not be apparent to the reader.}
% \textbf{Concern on use of jargon:}
\begin{itemize}
    \item Thank you for pointing out this point of confusion. We have revised our problem formulation section simplifying notation when possible and providing explanation for all symbols listed. In particular, we added clarification to the symbols presented, e.g., $(A,B)$ as the state-transition matrices, and have added definitions for terms the reader may not be familiar with, e.g., absolute continuity of a measure. 
\end{itemize}

\vspace{0.25cm}
\noindent
\emph{The example shown in Fig. 1 shows a pedestrian crossing the road, but this scenario was not studied in the paper. It would be better to show an example that was actually examined within the paper.}
% \textbf{Concern on Figure \ref{fig: Rollouts}:}
\begin{itemize}
    \item We have updated Figure \ref{fig: Rollouts} to demonstrate KLGame's policy guidance feature with a two-car interaction scenario from the Waymo Open Motion Dataset (WOMD) Interaction Validation set. We have also included trajectory snapshots from the racing example to illustrate the idea of policy blending. We hope that the revised figure helps demonstrate KLGame’s policy guidance and blending capabilities in challenging robotics tasks.  
\end{itemize}

\vspace{0.25cm}
\noindent
\emph{Section 2.C presents related work on multi-modal multi-agent motion prediction, though it is not clearly stated how the current work is different from the literature. It would be better to explain at the end of the section how the current work differs from these works (similar to the previous two sections).}
% \textbf{Concern on differentiating our approach from Multi-agent Multi-Modal Motion Prediction (Section II.C):}
\begin{itemize}
    \item We have stated at the end of each related work subsection how our method differs from the works listed.
\end{itemize}

\vspace{0.25cm}
\noindent
\emph{"Herein, we use $\neg i$ to denote..." - This sentence appears twice on page 4.}
\begin{itemize}
    \item We have fixed this issue. Thank you!
\end{itemize}

\vspace{0.25cm}
\noindent
\emph{In Table I, there are boldface entries for either the largest or smallest values except for the column "Dist (m)". Please apply boldface to the best-performing value as the others for consistency. Otherwise, it may appear as a metric that is not useful.}
% \textbf{Concern on bolding in Table \ref{tab: klgame_baseline_comparison}:}
\begin{itemize}
    \item In the original submission, we included the distance metric to record the minimum distance between the two agents as a measure of safety. However, since this metric is subsumed by the safe rate, we have removed it in the new version.
\end{itemize}


\vspace{0.25cm}
\noindent
\emph{In Fig. 4, it would be helpful to show a few intermediate values on both the x- and y-axis.}
% \textbf{Concern on showing the intermediate values in Figure \ref{fig: costs}:}
\begin{itemize}
    \item We have changed Figure \ref{fig: costs} to show the intermediate values.  
\end{itemize}


\vspace{0.25cm}
\noindent
\emph{In Fig. 9, the term "car" is used, but in Fig. 10 and 11, the term "agent" is used. Please use a consistent term throughout the paper.}
% \textbf{Concern on caption of Figure \ref{fig: waymax_scenario_3}:}
\begin{itemize}
    \item We have fixed the captions to ensure consistency.
\end{itemize}

\vspace{0.25cm}
\noindent
\emph{In Fig. 10, it states "As the agent 1 merges into the main road...". Isn't this supposed to be agent 0 that is merging into the main road? Agent 0 and 1 might be the other way around?}
\begin{itemize}
    \item We have fixed the numbers in the caption to refer to the correct agents.
\end{itemize}

\vspace{0.25cm}
\noindent
\emph{There is a typo in one subsection "...Planning Porblems".}
\begin{itemize}
    \item We have fixed this issue.
\end{itemize}

\vspace{0.25cm}
\noindent
\emph{It would be interesting to see the tunable parameter dynamically change if this can enable the agent to handle the situation better.}
% \textbf{Concern on tunable regularization parameters:}
\begin{itemize}
    \item Thank you for the suggestion. We note that devising a scheme to dynamically vary the tunable parameter optimally is nontrivial and beyond the scope of this paper. We are excited about the possibility of exploring this challenge for future work. 
\end{itemize}

\twocolumn
\newpage


